The Sound of Bounding-Boxes

In the task of audio-visual sound source separation, which leverages visual information for sound source separation, identifying objects in an image is a crucial step prior to separating the sound source. However, existing methods that assign sound on detected bounding boxes suffer from a problem that their approach heavily relies on pre-trained object detectors. Specifically, when using these existing methods, it is required to predetermine all the possible categories of objects that can produce sound and use an object detector applicable to all such categories. To tackle this problem, we propose a fully unsupervised method that learns to detect objects in an image and separate sound source simultaneously. As our method does not rely on any pre-trained detector, our method is applicable to arbitrary categories without any additional annotation. Furthermore, although being fully unsupervised, we found that our method performs comparably in separation accuracy.

==> fig/fig_solo_comparison.tex <==
\begin{figure*}[h]
    \scalebox{0.7}{
        \begin{tabular}{p{7.6em}p{7.6em}p{7.6em}p{0.04em}p{7.6em}p{7.6em}p{0.04em}p{7.6em}p{7.6em}}
        %\toprule
            %-------
        %-------
            \hfil \hfil 
            & \multicolumn{2}{c}{\qquad Example pair 1}
            & \hfil \hfil
            & \multicolumn{2}{c}{\qquad Example pair 2}
            & \hfil \hfil
            & \multicolumn{2}{c}{\qquad Example pair 3}
            	\tabularnewline
            	
        %-------
            % 1st
            \begin{minipage}{7.6em}
                \centering
                \scalebox{1}
                {Ours}
            \end{minipage} &
            % 2nd
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/acoustic_guitar-HGlIImajcRI+trumpet-zJIt_KdE3Jc/av1.png}}
            \end{minipage} &
            % 3rd
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/acoustic_guitar-HGlIImajcRI+trumpet-zJIt_KdE3Jc/av2.png}}
            \end{minipage} &
            % 4th
            \begin{minipage}{0.04em}
            \end{minipage} &
            
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/trumpet-Ba4ajAm0VDI+accordion-t_3Zm1PbydA/av1.png}}
            \end{minipage} &
            
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/trumpet-Ba4ajAm0VDI+accordion-t_3Zm1PbydA/av2.png}}
            \end{minipage} &
            \begin{minipage}{0.04em}
            \end{minipage} &
            
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/trumpet-aCi1P8Rymo4+violin-ZgGEuzLZw2E/av1.png}}
            \end{minipage} &
            % 4th
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/trumpet-aCi1P8Rymo4+violin-ZgGEuzLZw2E/av2.png}}
            \end{minipage} \vspace{0.001mm} \\
        %-------
        %-------
            %-------
            % 1st
            \begin{minipage}{7.6em}
                \centering
                \scalebox{1}
                {Co-Separating \cite{co_separating}}
            \end{minipage} &
            % 2nd
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/acoustic_guitar-HGlIImajcRI+trumpet-zJIt_KdE3Jc/av1_cosep.png}}
            \end{minipage} &
            % 3rd
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/acoustic_guitar-HGlIImajcRI+trumpet-zJIt_KdE3Jc/av2_cosep.png}}
            \end{minipage} &
            % 4th
            \begin{minipage}{0.04em}
            \end{minipage} &
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/trumpet-Ba4ajAm0VDI+accordion-t_3Zm1PbydA/av1_cosep.png}}
            \end{minipage} &
            
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/trumpet-Ba4ajAm0VDI+accordion-t_3Zm1PbydA/av2_cosep.png}}
            \end{minipage} &
            \begin{minipage}{0.04em}
            \end{minipage} &
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/trumpet-aCi1P8Rymo4+violin-ZgGEuzLZw2E/av1_cosep.png}}
            \end{minipage} &
            % 4th
            \begin{minipage}{7.6em}
                \centering
                \scalebox{0.390}
                {\includegraphics{png/solo_detected/trumpet-aCi1P8Rymo4+violin-ZgGEuzLZw2E/av2_cosep.png}}
            \end{minipage} \vspace{0.001mm} \\
            %-------
        %-------
        %-------
        %\bottomrule
        %-------
        \end{tabular}     }
    	\caption{The comparison of the detection result of our model and Co-separation in validation phase. As can be seen in the left image of the example pair 3, our model sometimes covers the larger region. In the same way, as can be seen in the left image of the example pair 2, our model sometimes covers the smaller region. These models are trained on the 7 categories that are available in Open Images V4 dataset.}
    \label{fig:solo_comparison} 
\end{figure*}
